Injectivity of polynomials over finite discrete dynamical systems

The analysis of observable phenomena (for instance, in biology or physics) allows the detection of dynamical behaviors and, conversely, starting from a desired behavior allows the design of objects exhibiting that behavior in engineering. The decomposition of dynamics into simpler subsystems allows us to simplify this analysis (or design). Here we focus on an algebraic approach to decomposition, based on alternative and synchronous execution as the sum and product operations; this gives rise to polynomial equations (with a constant side). In this article we focus on univariate, injective polynomials, giving a characterization in terms of the form of their coefficients and a polynomial-time algorithm for solving the associated equations.

==> algoPolyUnrolls.tex <==
Dans cette partie, nous allons des algorithmes polynomial pour calculer le $X$ tel $P(X) = B$ avec $P$ un polynôme à une variable et $B$ s'il existe.
Commençons par le cas des déroulements.
Pour ce faire, on pose le lemme suivant.

\begin{lemma}\label{lemme:baseAlgoRaisoEquaPoly}
	Soit $P(\tree{X}) = \sum_{i=1}^{n} \tree{A}_i\tree{X}^{k_i}$ avec $k_i < k_{i+1}$ un polynôme à une variable.
	Soit $d$ la plus grande des profondeurs des $\tree{A}_i$, $\tree{A}_\alpha$ le premier coefficient de $P$ qui a profondeur $d$, $\tree{a}_1$ le plus petit arbre de profondeur $d$ de $\tree{A}_\alpha$ et soit $\tree{B}$ une forêt.
	S'il existe $\tree{X}$ une forêt de profondeur au plus $d$ tel que $P(\tree{X}) = \tree{B}$ alors le plus petit arbre de $\tree{B}$ qui est divisible par $\tree{a}_1$ et dont le quotient admet une racine $k_\alpha$e est $\tree{a}_1 \tree{x}_1^{k_\alpha}$ avec $\tree{x}_1$ le plus petit arbre de $\tree{X}$.
\end{lemma}

\begin{proof}
	Supposons qu'il existe $\tree{X}$ une forêt de profondeur au plus $d$ tel que $P(\tree{X}) = \tree{B}$.
	On pose $\tree{b}$ le plus petit arbre de $\tree{B}$ qui est divisible par $\tree{a}_1$. 
	Supposons, par l'absurde, qu'il existe $\tree{y} \neq \tree{x}_1$ tel que $\tree{a}_1 \tree{y}^{k_\alpha} = \tree{b}$ et $\depth{y} \le d$.
	Donc comme $depth(\tree{x}_1) \le d$ par les lemmes 21 et 43 de \cite{1}, si $\tree{a}_1 \tree{x}_1^{k_\alpha} = \tree{b}$ alors $\tree{x}_1 = \tree{y}$, et puisque $\tree{b}$ est minimal, on déduit donc que $\tree{y} < \tree{x}_1$.
	Ainsi, comme $P(\tree{X}) = \tree{B}$, il existe $\ell$ et $i$ tel que $\tree{a}_\ell \tree{x}_i^{k_\ell} = \tree{b}$.
	Delà, deux cas sont possible.
	\begin{itemize}
		\item $\tree{a}_1 < \tree{a}_\ell$. 
		Donc $\tree{y}^{k_\alpha} > \tree{x}_i^{k_\ell}$.
		Mais comme $k_\ell \ge k_\alpha$, on déduit que $\tree{y} > \tree{x}_i \ge \tree{x}_1$. Contradiction.
		
		\item $\tree{a}_\ell \ge \tree{a}_1$. 
		Donc $\tree{a}_1 \tree{x}_1^{k_\ell} \le \tree{a}_\ell \tree{x}_1^{k_\ell} \le \tree{a}_\ell \tree{x}_i^{k_\ell} = \tree{a}_1 \tree{y}^{k_\alpha}$.
		Or comme $k_\ell \ge k_\alpha$, on a que $\tree{a}_1 \tree{x}_1^{k_\alpha} \le \tree{a}_1 \tree{x}_1^{k_\ell}$.
		Donc $\tree{x}_1^{k_\alpha} \le \tree{y}^{k_\alpha}$. 
		Donc $\tree{x}_1 \le \tree{y}$.
		Contradiction.
	\end{itemize}
\end{proof}
